Three-dimensional geometry and dust/gas ratios in massive star forming regions over the entire LMC as revealed by IRSF/SIRIUS survey

We derive the entire dust extinction (Av) map for the Large Magellanic Cloud (LMC) estimated from the color excess at near-infrared wavelengths. Using the percentile method we recently adopted to evaluate Av distribution along the line of sight, we derive the three-dimensional(3D)Av maps of the three massive star forming regions of N44, N79 and N11 based on the IRSF/SIRIUS point source catalog. The 3D AV maps are compared with the hydrogen column densities N(H) of three different velocity components where one is of the LMC disk velocity and the other two are of velocities lower than the disk velocity. As a result, we obtain 3D dust geometry suggesting that gas collision is on-going between the different velocity components. We also find difference in the timing of the gas collision between the massive star forming regions, which indicates that the gas collision in N44, N79 and N11 occurred later than that in 30 Doradus. In addition, difference by a factor of two in Av/N(H) is found between the velocity components for N44, while significant difference is not found for N79 and N11. From the 3D geometry and Av/N(H) in each star forming region, we suggest that the massive star formation in N44 was induced by an external trigger of tidal interaction between the LMC and the SMC, while that in N79 and N11 is likely to have been induced by internal triggers such as gas converging from the galactic spiral arm and expansion of a supershell although the possibility of tidal interaction cannot be ruled out.

==> 00README.XXX.tex <==
nohypertex
